RadarTrack: Enhancing Ego-Vehicle Speed Estimation with Single-chip mmWave Radar

In this work, we introduce RadarTrack, an innovative ego-speed estimation framework utilizing a single-chip millimeter-wave (mmWave) radar to deliver robust speed estimation for mobile platforms. Unlike previous methods that depend on cross-modal learning and computationally intensive Deep Neural Networks (DNNs), RadarTrack utilizes a novel phase-based speed estimation approach. This method effectively overcomes the limitations of conventional ego-speed estimation approaches which rely on doppler measurements and static surrondings. RadarTrack is designed for low-latency operation on embedded platforms, making it suitable for real-time applications where speed and efficiency are critical. Our key contributions include the introduction of a novel phase-based speed estimation technique solely based on signal processing and the implementation of a real-time prototype validated through extensive real-world evaluations. By providing a reliable and lightweight solution for ego-speed estimation, RadarTrack holds significant potential for a wide range of applications, including micro-robotics, augmented reality, and autonomous navigation.

==> tex/2primer.tex <==
\section{Primer}
Over the past decade, mmWave-based FMCW radars have become more accessible and widely used for various sensing applications~\cite{sen2024continuous, lien2016soli, sie2024radarize, sie2023batmobility, sen2023mmdrive, li2020capturing,wang2023long,vaidya2024exploiting}. These devices emit low-power radio signals and capture their reflections from the environment. By analyzing these reflections, the radar can estimate the distance, angle, and doppler shift of objects in its surroundings.

\subsection{Range Measurement}
In FMCW radars, the Intermediate Frequency (IF) is the difference between the transmitted and received frequencies and is proportional to the distance to the target. Given a transmitted chirp ($T_X$), a received chirp ($R_X$), and a transmission time $T_C$, the distance $d$ to an object can be calculated using $d = \frac{c}{2} \cdot \frac{T_C}{B} \cdot f_b$. Here, $f_b$ is the beat frequency, $c$ is the speed of light, and $\frac{T_C}{B}$ is the chirp slope $S$. A Range Fast Fourier Transform (Range-FFT) is applied to the IF signal to detect frequency peaks and calculate distances using the equation. This results in a one-dimensional array, or range profile, showing the received power across different distances.

\subsection{Range Resolution}
Range resolution is a radar's ability to distinguish between closely spaced objects. When objects are too close, the radar may not separate them. According to Fourier transform theory, increasing resolution requires extending the length of the IF signal, which necessitates increasing bandwidth. A longer IF signal allows the radar to resolve closely spaced frequency components. The range resolution $(d_{res})$ is given by $d_{res} = c/(2B)$, where $c$ is the speed of light and $B$ is the chirp bandwidth. Thus, higher bandwidths improve resolution. For example, a $4$ GHz chirp bandwidth provides a range resolution of about $3.75$ cm.

\subsection{Speed Measurement}
Speed measurement involves transmitting two chirps separated by $T_c$. Each reflected chirp is processed with Fast Fourier Transform (FFT) to detect range. The initial phase difference $\phi_0 = \frac{4\pi d}{\lambda}$ between the transmitted and received chirps, where $d$ is the distance, allows speed calculation. The phase difference $\Delta \phi$ is given by $\Delta \phi = 4\pi \frac{T_c}{\lambda}$. Speed $v$ is then calculated as $v = \frac{\lambda \Delta \phi}{4\pi T_c}$. The measurement is unambiguous if $|\Delta \phi| < \pi$, leading to a maximum measurable speed of $v_{max} = \frac{\lambda}{4T_c}$.

\subsection{Speed Resolution}\label{sec:vel_res}
Discrete Fourier transforms show that two frequencies $\omega_1$ and $\omega_2$ can be resolved if $\Delta \omega = \omega_2 - \omega_1 > \frac{2\pi}{N}$. Given $\Delta \omega = 4\pi \frac{T_c}{\lambda}$, the speed resolution $v_{\text{res}}$ is $v_{\text{res}} = \frac{\lambda}{2 N T_c}$. Typical the standard speed resolution of COTS mmWave radar is around 0.066m/s for number of chirps $N = 128 \times 3$ (number of transmitters)~\cite{li2021signal, sie2024radarize, kramer2020radar}. Thus all these previous works on ego-speed estimation can't deal with speeds lower than this resolution.
